Network-Side Digital Contact Tracing on a Large University Campus

We describe a study conducted at a large public university campus in the United States which shows the efficacy of network log information for digital contact tracing and prediction of COVID-19 cases. Over the period of January 18, 2021 to May 7, 2021, more than 216 million client-access-point associations were logged across more than 11,000 wireless access points (APs). The association information was used to find potential contacts for approximately 30,000 individuals. Contacts are determined using an AP colocation algorithm, which supposes contact when two individuals connect to the same WiFi AP at approximately the same time. The approach was validated with a truth set of 350 positive COVID-19 cases inferred from the network log data by observing associations with APs in isolation residence halls reserved for individuals with a confirmed (clinical) positive COVID-19 test result. The network log data and AP-colocation have a predictive value of greater than 10%; more precisely, the contacts of an individual with a confirmed positive COVID-19 test have greater than a 10\% chance of testing positive in the following 7 days (compared with a 0.79% chance when chosen at random, a relative risk ratio of 12.6). Moreover, a cumulative exposure score is computed to account for exposure to multiple individuals that test positive. Over the duration of the study, the cumulative exposure score predicts positive cases with a true positive rate of 16.5% and missed detection rate of 79% at a specified operating point.

==> deleted.tex <==
\subsection{Truth Set}

In lieu of tracing devices to personal identities and COVID-19 test status, we decided to use campus policies and device behavior to infer status. The occupancy count of the isolation dorms provide a basis for comparison against which we can validate counts and device:person ratios obtained via analysis of the Wi-Fi network. Since these isolation dorms have been reserved to house only COVID-19 positive students, we can infer a positive COVID-19 infection status from devices that appear to relocate to the isolation dorms for a period approximately matching the suggested isolation period. We use this information to identify a set of plausible positive cases to test our contact tracing algorithm. Importantly, only students who were living in residence halls and test positive are required to move into the isolation dorms. We therefore use a similar process to identify those devices that plausibly belong to students residing in on-campus housing. Ultimately, our digital contact tracing approach can still identify contacts among off-campus residents and non-students, but we are not able to use Wi-Fi data from the isolation dorms to infer their health status.

\subsection{Inferring Dorm Residents}

Our two goals are to find devices that belong to dorm residents and for residents with more than one device, identify the device most likely to be carried on the person, ie. the mobile phone. A study of multi-device user behavior~\cite{trivedi2020empirical} suggests distinguishing devices based on network behavior at different hours of the day. Always-on devices, of which phones are quite common, remain active on the WiFi network in the early hours of the morning, when other devices such as laptops and entertainment devices are likely to be in a low power, non-transmitting state. Additionally, we expect based on human behavior, if we choose an appropriate time window, we can minimize the presence of visitors and employees to identify devices that plausibly belong to people who reside in the dorm.

First, we look at the feasibility of estimating building occupancy in the COVID-19 isolation dorms. For these five dorms, we have ground truth daily resident counts from the campus health authorities. We frame this as an optimization problem of choosing the best hour of the day to use WiFi logs to predict the number of residents in a dorm. If we measure device activity during daytime hours, we expect a noisy result that counts employee devices and other devices owned by the residents in addition to their phones. We selected the time window of 4:00-5:00 AM because it minimizes the prediction error on the true number of building residents. Figure~\ref{fig:morning-counts} shows daily counts of residents in five dorms as reported by the university and as predicted by counting the number of detected devices between 4:00 and 5:00 AM. Figure~\ref{fig:mse-residents} shows how we arrived at the choice of this time window for predicting residents as the minimum mean squared error estimator out of the 24 one-hour time windows we tested. Compared to the general problem of predicting building occupancy from WiFi activity, device and user behavior makes dorm residency an easier problem.

After that finding early morning device activity is strongly correlated with building resident counts, we apply the same approach to all of the campus residence halls. Although we do not have ground truth numbers for Spring semester residents, we are able to find the reported capacity of each dorm from the university housing webpages. Define $N_h$ as the capacity of residence hall $h$. We scan the network logs for devices detected in each residence hall between 4:00 and 5:00 AM and count the number of days in which a device is detected in a given hall. For each hall $h$, we sort from the highest to lowest detection counts and select the top $N_h$ devices as probable residents in that building.

We use the aggregate set of resident devices as the population of interest for the rest of this study and discard non-resident devices. Although we are able to compute AP colocation metrics for non-resident devices and perform digital contact tracing, we are only able to evaluate efficacy for contact tracing in the COVID-19 pandemic on the subset of devices that belong to university housing residents. This is made possible by the campus policy of requiring housing residents to move into dedicated isolation housing units after testing positive for COVID-19.
